Origami Inspired Reconfigurable Antenna for Wireless Communication Systems

This paper presents the design, fabrication, and experimental validation of an origami-inspired reconfigurable antenna. The proposed antenna can operate as a monopole or an inverted-L antenna, by changing its configuration. Doing so changes its operational frequency, principal radiation mode, and directivity. Measurements show that the antenna is able to change its resonance frequency from 750 MHz to 920 MHz---equivalent to 22.6\% frequency shift. Simulations are carried out to compare the radiation characteristics of the antenna (gain and radiation pattern) in both configurations. The results validate that the antenna has a reconfigurable bandwidth, which enables a better channel characterization for RF systems.

==> Origami_Ant <==
% This file was created with JabRef 2.10.
% Encoding: Cp1252


@Article{liu2015origami,
  Title                    = {An origami reconfigurable axial-mode bifilar helical antenna},
  Author                   = {Liu, Xueli and Yao, Shun and Cook, Benjamin S and Tentzeris, Manos M and Georgakopoulos, Stavros V},
  Journal                  = {IEEE Transactions on Antennas and Propagation},
  Year                     = {2015},
  Number                   = {12},
  Pages                    = {5897--5903},
  Volume                   = {63},

  Publisher                = {IEEE}
}

@InProceedings{liu2015reconfigurable,
  Title                    = {Reconfigurable origami equiangular conical spiral antenna},
  Author                   = {Liu, Xueli and Yao, Shun and Georgakopoulos, Stavros V},
  Booktitle                = {Antennas and Propagation \& USNC/URSI National Radio Science Meeting, 2015 IEEE International Symposium on},
  Year                     = {2015},
  Organization             = {IEEE},
  Pages                    = {2263--2264}
}

@InProceedings{liu2014reconfigurable,
  Title                    = {Reconfigurable helical antenna based on an origami structure for wireless communication system},
  Author                   = {Liu, XueLi and Yao, Shun and Georgakopoulos, Stavros V and Cook, Benjamin S and Tentzeris, Manos M},
  Booktitle                = {Microwave Symposium (IMS), 2014 IEEE MTT-S International},
  Year                     = {2014},
  Organization             = {IEEE},
  Pages                    = {1--4}
}

@Article{shah2017low,
  Title                    = {Low-Cost Circularly Polarized Origami Antenna},
  Author                   = {Shah, Syed Imran Hussain and Tentzeris, Manos M and Lim, Sungjoon},
  Journal                  = {IEEE Antennas and Wireless Propagation Letters},
  Year                     = {2017},
  Pages                    = {2026--2029},
  Volume                   = {16},

  Publisher                = {IEEE}
}

@InProceedings{yao2014novel,
  Title                    = {A novel reconfigurable origami accordion antenna},
  Author                   = {Yao, Shun and Georgakopoulos, Stavros V and Cook, Benjamin and Tentzeris, Manos},
  Booktitle                = {Microwave Symposium (IMS), 2014 IEEE MTT-S International},
  Year                     = {2014},
  Organization             = {IEEE},
  Pages                    = {1--4}
}

@InProceedings{yao2015mode,
  Title                    = {A mode reconfigurable Nojima origami antenna},
  Author                   = {Yao, Shun and Liu, Xueli and Georgakopoulos, Stavros V},
  Booktitle                = {Antennas and Propagation \& USNC/URSI National Radio Science Meeting, 2015 IEEE International Symposium on},
  Year                     = {2015},
  Organization             = {IEEE},
  Pages                    = {2237--2238}
}

@InProceedings{yao2016polarization,
  Title                    = {Polarization switchable origami helical antenna},
  Author                   = {Yao, Shun and Liu, Xueli and Georgakopoulos, Stavros V and Schamp, Ray},
  Booktitle                = {Antennas and Propagation (APSURSI), 2016 IEEE International Symposium on},
  Year                     = {2016},
  Organization             = {IEEE},
  Pages                    = {1667--1668}
}

@InProceedings{yao2014novel2,
  Title                    = {A novel reconfigurable origami spring antenna},
  Author                   = {Yao, Shun and Liu, Xueli and Georgakopoulos, Stavros V and Tentzeris, Manos M},
  Booktitle                = {Antennas and Propagation Society International Symposium (APSURSI), 2014 IEEE},
  Year                     = {2014},
  Organization             = {IEEE},
  Pages                    = {374--375}
}


